IceCat-1: the IceCube Event Catalog of Alert Tracks

We present a catalog of likely astrophysical neutrino track-like events from the IceCube Neutrino Observatory. IceCube began reporting likely astrophysical neutrinos in 2016 and this system was updated in 2019. The catalog presented here includes events that were reported in real-time since 2019, as well as events identified in archival data samples starting from 2011. We report 275 neutrino events from two selection channels as the first entries in the catalog, the IceCube Event Catalog of Alert Tracks, which will see ongoing extensions with additional alerts. The gold and bronze alert channels respectively provide neutrino candidates with 50\% and 30\% probability of being astrophysical, on average assuming an astrophysical neutrino power law energy spectral index of 2.19. For each neutrino alert, we provide the reconstructed energy, direction, false alarm rate, probability of being astrophysical in origin, and likelihood contours describing the spatial uncertainty in the alert's reconstructed location. We also investigate a directional correlation of these neutrino events with gamma-ray and X-ray catalogs including 4FGL, 3HWC, TeVCat and Swift-BAT.

==> catalog.tex <==
IC20110514 & $138.47^{6.68}_{3.78}$ & $-1.94^{0.97}_{1.12}$ & 187 & $0.51$ & 4FGL J0914.1-0202 (0.12) & 3FHL J0909.7-0231 (1.18) & -- (--) & -- (--) & -- (--) \\
IC20110610 & $272.55^{1.67}_{2.42}$ & $35.64^{1.30}_{1.05}$ & 294 & $0.75$ & 4FGL J1808.8+3522 (0.37) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110616 & $71.15^{1.41}_{2.07}$ & $5.38^{0.79}_{0.90}$ & 109 & $0.26$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110714 & $68.20^{0.31}_{1.10}$ & $40.67^{0.44}_{0.44}$ & 72 & $0.78$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110726 & $151.08^{1.19}_{1.71}$ & $6.99^{0.98}_{0.83}$ & 160 & $0.40$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110807 & $336.80^{1.36}_{1.98}$ & $1.53^{0.93}_{0.78}$ & 108 & $0.27$ & 4FGL J2226.6+0210 (0.65) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110818 & $332.45^{0.97}_{1.23}$ & $-2.09^{0.93}_{0.90}$ & 123 & $0.34$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110902 & $9.76^{2.86}_{1.32}$ & $7.59^{0.87}_{0.86}$ & 243 & $0.61$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110907 & $196.08^{3.91}_{2.68}$ & $9.40^{1.55}_{1.06}$ & 186 & $0.51$ & 4FGL J1301.6+0834 (1.06) & -- (--) & -- (--) & -- (--) &    SWIFT J1310.7+08 (1.78) \\
IC20110929 & $121.45^{1.34}_{1.29}$ & $50.04^{0.24}_{0.15}$ & 158 & $0.52$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20110930 & $267.01^{1.19}_{1.14}$ & $-4.44^{0.60}_{0.79}$ & 160 & $0.43$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20111012 & $172.13^{1.40}_{1.39}$ & $44.70^{0.79}_{0.45}$ & 115 & $0.43$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20111120 & $26.06^{1.89}_{3.16}$ & $9.82^{1.40}_{1.36}$ & 159 & $0.42$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20111120 & $356.84^{0.53}_{0.62}$ & $-11.99^{0.23}_{0.27}$ & 4969 & $0.29$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20111208 & $165.19^{7.03}_{4.13}$ & $38.49^{3.67}_{3.49}$ & 123 & $0.45$ & 4FGL J1101.5+3904 (0.6) & 3FHL J1104.4+3812 (0.78) & 3HWC J1104+381 (0.8) & Markarian 421 (0.76) &    SWIFT J1104.4+38 (0.77) \\
IC20111209 & $99.98^{1.19}_{2.02}$ & $20.42^{1.60}_{2.02}$ & 108 & $0.34$ & -- (--) & -- (--) & 3HWC J0633+191 (1.95) & -- (--) & -- (--) \\
IC20111213 & $247.85^{1.71}_{1.58}$ & $0.56^{1.46}_{1.42}$ & 164 & $0.41$ & 4FGL J1638.0+0042 (1.67) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20111216 & $36.74^{1.80}_{2.24}$ & $18.88^{2.46}_{2.82}$ & 891 & $0.95$ & 4FGL J0224.9+1843 (0.51) & -- (--) & -- (--) & -- (--) &    SWIFT J0225.0+18 (0.46) \\
IC20111218 & $26.85^{3.69}_{4.66}$ & $7.03^{4.04}_{5.20}$ & 157 & $0.40$ & 4FGL J0151.0+0539 (1.65) & 3FHL J0151.0+0539 (1.64) & -- (--) & -- (--) & -- (--) \\
IC20120301 & $237.96^{0.53}_{0.62}$ & $18.76^{0.47}_{0.51}$ & 433 & $0.82$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120426 & $183.56^{2.15}_{2.02}$ & $0.52^{0.86}_{0.71}$ & 109 & $0.27$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120501 & $165.37^{7.01}_{5.36}$ & $-71.51^{3.53}_{2.68}$ & 85 & $0.46$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120515 & $198.94^{1.71}_{1.41}$ & $32.00^{0.97}_{1.09}$ & 194 & $0.61$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120523 & $171.08^{0.66}_{1.41}$ & $26.44^{0.46}_{0.37}$ & 213 & $0.53$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120523 & $343.78^{4.92}_{4.48}$ & $15.48^{2.38}_{1.54}$ & 168 & $0.49$ & 4FGL J2253.9+1609 (0.72) & 3FHL J2253.9+1608 (0.72) & -- (--) & -- (--) &    SWIFT J2253.9+16 (0.73) \\
IC20120529 & $176.48^{6.64}_{5.93}$ & $22.87^{2.70}_{1.77}$ & 126 & $0.42$ & 4FGL J1150.4+2418 (1.76) & 3FHL J1150.3+2418 (1.75) & -- (--) & -- (--) &    SWIFT J1141.3+21 (1.45) \\
IC20120601 & $119.31^{2.02}_{0.92}$ & $14.79^{0.62}_{0.73}$ & 137 & $0.40$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120605 & $152.58^{1.89}_{2.42}$ & $36.38^{1.54}_{1.47}$ & 107 & $0.39$ & 4FGL J1011.6+3600 (0.45) & 3FHL J1006.9+3455 (1.61) & -- (--) & -- (--) &    SWIFT J1008.6+37 (1.23) \\
IC20120611 & $39.95^{0.26}_{0.26}$ & $-15.09^{0.19}_{0.31}$ & 9220 & $0.24$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120807 & $330.07^{0.83}_{0.83}$ & $1.42^{0.60}_{0.45}$ & 373 & $0.74$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120916 & $182.24^{1.36}_{1.71}$ & $3.88^{0.67}_{0.82}$ & 174 & $0.44$ & 4FGL J1204.8+0407 (1.06) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20120922 & $70.62^{1.49}_{1.27}$ & $19.79^{0.91}_{0.71}$ & 143 & $0.43$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20121011 & $205.14^{0.66}_{0.70}$ & $-2.28^{0.52}_{0.56}$ & 481 & $0.84$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20121026 & $169.80^{1.32}_{1.41}$ & $27.91^{0.85}_{0.88}$ & 961 & $0.93$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20121103 & $123.18^{0.92}_{0.97}$ & $6.05^{0.64}_{0.56}$ & 112 & $0.28$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20121115 & $225.70^{1.01}_{1.19}$ & $8.88^{0.94}_{0.95}$ & 116 & $0.32$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130125 & $7.67^{6.46}_{5.92}$ & $74.14^{3.36}_{2.82}$ & 165 & $0.53$ & 4FGL J0028.1+7505 (0.97) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130125 & $280.46^{1.89}_{2.33}$ & $-1.90^{0.93}_{0.82}$ & 114 & $0.31$ & 4FGL J1847.2-0141 (1.37) & -- (--) & 3HWC J1847-017 (1.5) & -- (--) & -- (--) \\
IC20130127 & $352.97^{1.32}_{1.01}$ & $-1.98^{0.97}_{0.90}$ & 235 & $0.61$ & 4FGL J2333.4-0133 (0.58) & -- (--) & -- (--) & -- (--) &    SWIFT J2330.5-02 (0.6) \\
IC20130208 & $48.38^{0.31}_{0.31}$ & $-13.32^{0.23}_{0.23}$ & 2268 & $0.32$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130316 & $303.41^{2.98}_{3.55}$ & $54.68^{1.77}_{1.59}$ & 105 & $0.38$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J2006.5+56 (1.93) \\
IC20130318 & $13.45^{0.79}_{0.88}$ & $20.62^{1.44}_{0.99}$ & 106 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130408 & $167.83^{2.64}_{3.96}$ & $20.66^{1.28}_{0.99}$ & 65 & $0.53$ & 4FGL J1117.0+2013 (1.42) & 3FHL J1117.0+2014 (1.41) & -- (--) & -- (--) &    SWIFT J1114.3+20 (0.71) \\
IC20130408 & $7.38^{4.88}_{8.04}$ & $4.22^{4.73}_{3.58}$ & 163 & $0.40$ & 4FGL J0030.4+0451 (0.68) & 3FHL J0022.4+0607 (2.59) & -- (--) & -- (--) & -- (--) \\
IC20130409 & $163.56^{2.68}_{2.50}$ & $29.44^{4.38}_{3.46}$ & 115 & $0.41$ & 4FGL J1058.6+2817 (1.5) & -- (--) & -- (--) & GB6 J1058+2817 (1.48) & -- (--) \\
IC20130508 & $337.76^{3.21}_{2.02}$ & $26.24^{2.69}_{1.90}$ & 140 & $0.45$ & 4FGL J2223.0+2704 (1.97) & -- (--) & -- (--) & -- (--) &    SWIFT J2237.0+25 (1.35) \\
IC20130509 & $317.50^{1.76}_{1.85}$ & $2.09^{1.19}_{1.34}$ & 105 & $0.25$ & 4FGL J2104.7+0108 (1.63) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130519 & $45.35^{3.12}_{1.49}$ & $23.85^{1.15}_{0.89}$ & 110 & $0.36$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130531 & $164.18^{2.42}_{2.15}$ & $6.32^{1.32}_{1.27}$ & 143 & $0.35$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130627 & $93.74^{1.01}_{1.14}$ & $14.17^{1.23}_{1.04}$ & 851 & $0.94$ & 4FGL J0615.9+1416 (0.26) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130627 & $155.35^{3.87}_{2.37}$ & $3.73^{1.72}_{1.42}$ & 122 & $0.31$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130711 & $77.87^{2.59}_{1.19}$ & $-2.43^{1.34}_{1.12}$ & 165 & $0.43$ & 4FGL J0515.5-0125 (1.44) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130731 & $122.87^{2.29}_{4.35}$ & $6.32^{3.24}_{2.40}$ & 122 & $0.32$ & 4FGL J0812.5+0711 (0.92) & -- (--) & -- (--) & -- (--) &    SWIFT J0814.3+04 (2.08) \\
IC20130801 & $214.98^{4.35}_{4.00}$ & $7.75^{1.24}_{1.20}$ & 110 & $0.28$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J1419.1+07 (0.26) \\
IC20130804 & $129.02^{1.14}_{1.54}$ & $13.36^{1.08}_{1.68}$ & 113 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130808 & $26.59^{1.14}_{1.23}$ & $9.22^{0.91}_{0.87}$ & 111 & $0.29$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20130822 & $91.32^{1.19}_{1.19}$ & $0.56^{0.78}_{0.63}$ & 115 & $0.30$ & 4FGL J0604.9-0000 (0.57) & 3FHL J0604.9+0000 (0.56) & -- (--) & -- (--) & -- (--) \\
IC20130907 & $130.17^{0.48}_{0.31}$ & $-10.54^{0.27}_{0.30}$ & 890 & $0.32$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20131014 & $32.92^{0.88}_{0.70}$ & $10.28^{0.42}_{0.57}$ & 293 & $0.67$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20131023 & $301.90^{1.01}_{1.05}$ & $11.61^{1.14}_{1.29}$ & 211 & $0.59$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20131108 & $342.73^{1.54}_{1.58}$ & $41.81^{1.40}_{0.89}$ & 153 & $0.50$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20131112 & $129.24^{0.26}_{0.26}$ & $-17.27^{0.16}_{0.16}$ & 7006 & $0.27$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20131124 & $285.16^{2.20}_{1.54}$ & $19.47^{1.43}_{1.46}$ & 180 & $0.55$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20131204 & $288.98^{1.10}_{0.83}$ & $-14.21^{0.77}_{1.31}$ & 259 & $0.20$ & 4FGL J1916.7-1516 (1.08) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140101 & $192.26^{2.07}_{2.37}$ & $-2.69^{1.01}_{0.71}$ & 200 & $0.56$ & 4FGL J1251.3-0201 (0.88) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140103 & $37.90^{25.61}_{27.30}$ & $78.97^{5.86}_{9.97}$ & 125 & $0.42$ & 4FGL J0226.9+7744 (1.25) & 3FHL J0233.9+8042 (1.75) & -- (--) & -- (--) &    SWIFT J0306.4+76 (3.15) \\
IC20140108 & $344.66^{0.53}_{0.48}$ & $1.57^{0.37}_{0.34}$ & 214 & $0.69$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140109 & $293.12^{0.79}_{1.19}$ & $33.02^{0.45}_{0.53}$ & 924 & $0.93$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J1933.9+32 (0.31) \\
IC20140114 & $337.59^{0.57}_{0.92}$ & $0.71^{0.97}_{0.86}$ & 54 & $0.34$ & 4FGL J2227.9+0036 (0.61) & 3FHL J2227.8+0036 (0.63) & -- (--) & -- (--) & -- (--) \\
IC20140122 & $138.82^{3.52}_{10.11}$ & $37.45^{1.95}_{2.09}$ & 131 & $0.46$ & 4FGL J0916.7+3856 (1.53) & -- (--) & -- (--) & -- (--) &    SWIFT J0920.1+37 (0.99) \\
IC20140122 & $220.29^{8.94}_{8.37}$ & $-86.07^{0.59}_{0.64}$ & 374 & $0.82$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140203 & $349.58^{2.64}_{2.55}$ & $-13.55^{1.15}_{1.73}$ & 685 & $0.13$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140213 & $202.59^{4.79}_{3.21}$ & $13.06^{2.31}_{2.52}$ & 140 & $0.39$ & 4FGL J1326.1+1232 (1.14) & 3FHL J1323.9+1405 (1.87) & -- (--) & -- (--) & -- (--) \\
IC20140223 & $118.83^{11.87}_{11.87}$ & $32.58^{5.68}_{9.83}$ & 119 & $0.43$ & 4FGL J0752.2+3313 (0.92) & 3FHL J0809.7+3457 (3.82) & -- (--) & -- (--) &    SWIFT J0749.8+33 (1.82) \\
IC20140307 & $308.06^{2.68}_{4.61}$ & $32.93^{2.71}_{3.23}$ & 109 & $0.40$ & 4FGL J2028.3+3331 (1.01) & 3FHL J2027.0+3343 (1.35) & 3HWC J2023+324 (1.95) & -- (--) &    SWIFT J2025.5+33 (1.62) \\
IC20140324 & $225.70^{5.67}_{4.65}$ & $51.06^{4.00}_{2.87}$ & 109 & $0.40$ & 4FGL J1456.0+5051 (1.08) & 3FHL J1454.5+5124 (1.34) & -- (--) & -- (--) & -- (--) \\
IC20140410 & $2.11^{151.51}_{58.92}$ & $81.22^{8.00}_{6.94}$ & 246 & $0.63$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0017.1+81 (0.5) \\
IC20140411 & $146.95^{3.12}_{3.12}$ & $15.91^{2.89}_{2.62}$ & 156 & $0.45$ & 4FGL J0949.2+1749 (1.95) & -- (--) & -- (--) & -- (--) &    SWIFT J0947.3+13 (2.15) \\
IC20140420 & $6.28^{7.03}_{5.89}$ & $16.57^{4.77}_{5.11}$ & 163 & $0.49$ & 4FGL J0023.9+1603 (0.58) & 3FHL J0035.2+1514 (2.78) & -- (--) & -- (--) &    SWIFT J0029.2+13 (3.42) \\
IC20140503 & $162.30^{6.91}_{11.26}$ & $46.57^{5.41}_{5.11}$ & 109 & $0.40$ & 4FGL J1053.7+4930 (3.03) & 3FHL J1053.6+4930 (3.03) & -- (--) & -- (--) &    SWIFT J1107.3+48 (3.49) \\
IC20140603 & $9.71^{0.62}_{0.88}$ & $7.56^{0.53}_{0.83}$ & 152 & $0.38$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140609 & $106.26^{2.68}_{2.15}$ & $1.31^{1.05}_{0.86}$ & 459 & $0.81$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140611 & $110.65^{0.53}_{0.62}$ & $11.45^{0.19}_{0.19}$ & 5960 & $1.00$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140704 & $157.07^{4.69}_{4.64}$ & $53.62^{3.35}_{3.48}$ & 150 & $0.50$ & 4FGL J1043.0+5316 (2.22) & 3FHL J1031.3+5053 (2.77) & -- (--) & -- (--) &    SWIFT J1033.8+52 (1.07) \\
IC20140705 & $25.88^{1.85}_{2.99}$ & $2.54^{1.79}_{1.75}$ & 212 & $0.56$ & 4FGL J0138.5+0300 (1.33) & 3FHL J0148.6+0127 (1.68) & -- (--) & -- (--) & -- (--) \\
IC20140707 & $240.86^{3.08}_{2.07}$ & $14.17^{1.54}_{1.65}$ & 167 & $0.48$ & 4FGL J1606.2+1346 (0.8) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140713 & $0.79^{1.14}_{1.19}$ & $15.60^{0.89}_{0.66}$ & 134 & $0.39$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140721 & $101.82^{6.77}_{6.86}$ & $-32.89^{5.23}_{8.08}$ & 157 & $0.56$ & 4FGL J0649.5-3139 (1.32) & 3FHL J0649.5-3138 (1.33) & -- (--) & PKS 0625-35 (4.94) &    SWIFT J0701.3-32 (2.94) \\
IC20140820 & $271.45^{3.43}_{1.80}$ & $1.87^{1.42}_{1.46}$ & 108 & $0.27$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140923 & $169.72^{0.70}_{0.83}$ & $-1.60^{0.52}_{0.30}$ & 209 & $0.24$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20140927 & $50.89^{3.91}_{5.14}$ & $-0.63^{1.49}_{1.42}$ & 182 & $0.48$ & 4FGL J0323.7-0111 (0.56) & 3FHL J0323.6-0109 (0.54) & -- (--) & -- (--) & -- (--) \\
IC20141012 & $63.85^{2.24}_{1.36}$ & $3.21^{0.90}_{1.08}$ & 173 & $0.44$ & 4FGL J0412.3+0239 (0.94) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20141110 & $253.43^{0.83}_{1.10}$ & $6.43^{0.71}_{0.68}$ & 113 & $0.29$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20141114 & $221.48^{4.53}_{2.29}$ & $28.00^{2.31}_{2.30}$ & 110 & $0.38$ & 4FGL J1449.5+2746 (0.84) & 3FHL J1449.5+2745 (0.84) & -- (--) & -- (--) &    SWIFT J1445.6+27 (0.98) \\
IC20141208 & $246.36^{1.76}_{1.89}$ & $17.23^{1.29}_{1.09}$ & 109 & $0.33$ & 4FGL J1626.4+1820 (1.13) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20141210 & $318.12^{2.33}_{1.93}$ & $1.57^{1.57}_{1.72}$ & 154 & $0.37$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20141221 & $179.08^{0.88}_{1.10}$ & $-1.94^{0.71}_{0.82}$ & 134 & $0.35$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150102 & $318.74^{3.96}_{1.27}$ & $2.91^{0.34}_{0.49}$ & 126 & $0.32$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150104 & $272.11^{1.71}_{1.54}$ & $28.76^{2.41}_{1.86}$ & 133 & $0.45$ & 4FGL J1807.1+2822 (0.48) & 3FHL J1809.8+2911 (0.52) & -- (--) & -- (--) & -- (--) \\
IC20150118 & $152.53^{1.54}_{2.72}$ & $4.33^{0.71}_{0.86}$ & 156 & $0.37$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150119 & $286.92^{1.36}_{1.27}$ & $6.43^{0.60}_{0.53}$ & 140 & $0.35$ & 4FGL J1906.2+0631 (0.37) & 3FHL J1907.9+0602 (0.4) & 3HWC J1908+063 (0.14) & LHAASO J1908+062 (0.15) & -- (--) \\
IC20150120 & $95.89^{1.19}_{1.36}$ & $14.13^{0.50}_{0.50}$ & 113 & $0.34$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150127 & $100.37^{1.36}_{1.63}$ & $4.59^{0.79}_{0.67}$ & 293 & $0.66$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150129 & $358.51^{3.91}_{6.55}$ & $6.39^{3.16}_{3.67}$ & 130 & $0.33$ & 4FGL J2349.4+0534 (1.41) & 3FHL J2346.6+0705 (1.95) & -- (--) & -- (--) &    SWIFT J2343.9+05 (2.62) \\
IC20150224 & $237.75^{8.26}_{2.26}$ & $55.11^{3.38}_{3.03}$ & 106 & $0.38$ & 4FGL J1553.1+5438 (0.56) & 3FHL J1558.8+5626 (1.73) & -- (--) & -- (--) & -- (--) \\
IC20150313 & $127.05^{1.76}_{2.07}$ & $-3.36^{0.75}_{0.75}$ & 107 & $0.29$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150428 & $31.07^{4.04}_{6.42}$ & $15.02^{1.94}_{1.42}$ & 109 & $0.32$ & 4FGL J0204.8+1513 (0.26) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150515 & $91.49^{0.92}_{0.75}$ & $12.14^{0.53}_{0.50}$ & 401 & $0.77$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150526 & $139.79^{2.46}_{2.99}$ & $-1.49^{0.90}_{1.01}$ & 108 & $0.28$ & 4FGL J0914.1-0202 (1.36) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150601 & $333.37^{2.42}_{1.71}$ & $9.63^{1.21}_{1.17}$ & 106 & $0.27$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150609 & $49.53^{1.10}_{1.10}$ & $0.30^{0.45}_{0.82}$ & 118 & $0.31$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150609 & $245.43^{1.67}_{1.23}$ & $0.22^{1.04}_{0.93}$ & 116 & $0.30$ & 4FGL J1625.1-0020 (1.03) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150625 & $71.89^{4.35}_{4.70}$ & $0.86^{2.39}_{1.83}$ & 112 & $0.29$ & 4FGL J0442.6-0017 (1.69) & 3FHL J0442.7-0018 (1.69) & -- (--) & -- (--) & -- (--) \\
IC20150625 & $306.43^{2.02}_{2.02}$ & $19.08^{0.91}_{1.18}$ & 154 & $0.46$ & 4FGL J2030.9+1935 (1.34) & 3FHL J2031.0+1936 (1.35) & -- (--) & -- (--) & -- (--) \\
IC20150714 & $326.29^{1.49}_{1.32}$ & $26.36^{1.89}_{2.19}$ & 439 & $0.84$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150809 & $221.75^{0.31}_{0.26}$ & $-17.15^{0.23}_{0.16}$ & 11667 & $0.20$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150812 & $317.59^{5.10}_{4.66}$ & $30.09^{2.31}_{2.43}$ & 125 & $0.44$ & 4FGL J2115.4+2932 (1.24) & 3FHL J2115.2+2933 (1.19) & -- (--) & -- (--) & -- (--) \\
IC20150812 & $328.27^{0.75}_{0.88}$ & $6.17^{0.49}_{0.53}$ & 508 & $0.83$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150823 & $325.90^{3.47}_{4.17}$ & $-2.35^{2.61}_{2.09}$ & 133 & $0.35$ & 4FGL J2148.9-0121 (1.66) & 3FHL J2134.2-0152 (2.38) & -- (--) & -- (--) & -- (--) \\
IC20150831 & $54.76^{0.92}_{0.92}$ & $34.00^{1.13}_{1.21}$ & 181 & $0.58$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150904 & $133.77^{0.53}_{0.88}$ & $28.08^{0.51}_{0.55}$ & 302 & $0.74$ & 4FGL J0854.0+2753 (0.3) & 3FHL J0854.1+2752 (0.29) & -- (--) & -- (--) & -- (--) \\
IC20150914 & $129.68^{1.89}_{2.59}$ & $30.35^{1.88}_{1.29}$ & 120 & $0.43$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0840.2+29 (0.63) \\
IC20150918 & $49.83^{2.50}_{3.74}$ & $-2.95^{1.35}_{1.34}$ & 105 & $0.28$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0324.9-03 (1.41) \\
IC20150919 & $279.54^{1.76}_{2.29}$ & $30.35^{2.19}_{1.50}$ & 228 & $0.67$ & 4FGL J1836.4+3137 (1.32) & 3FHL J1836.4+3137 (1.32) & -- (--) & -- (--) &    SWIFT J1832.2+31 (1.7) \\
IC20150923 & $103.23^{0.70}_{1.14}$ & $3.96^{0.60}_{0.75}$ & 216 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20150926 & $194.55^{0.79}_{1.23}$ & $-4.56^{0.93}_{0.64}$ & 216 & $0.30$ & 4FGL J1258.7-0452 (0.34) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20151013 & $178.72^{1.11}_{1.15}$ & $52.37^{1.11}_{1.11}$ & 156 & $0.52$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20151017 & $197.53^{2.46}_{2.72}$ & $19.95^{3.01}_{2.29}$ & 321 & $0.75$ & 4FGL J1311.8+2057 (1.09) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20151114 & $76.16^{1.36}_{1.36}$ & $12.71^{0.65}_{0.73}$ & 1124 & $0.96$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20151122 & $262.05^{0.88}_{1.05}$ & $-2.24^{0.63}_{0.67}$ & 253 & $0.64$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160104 & $79.41^{0.83}_{0.75}$ & $5.00^{0.86}_{0.97}$ & 217 & $0.57$ & 4FGL J0515.9+0537 (0.75) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160128 & $263.76^{1.10}_{1.80}$ & $-14.90^{1.08}_{1.20}$ & 583 & $0.15$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160225 & $311.87^{2.18}_{1.78}$ & $60.06^{1.65}_{1.37}$ & 188 & $0.60$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160307 & $91.32^{7.08}_{8.66}$ & $10.47^{2.74}_{4.45}$ & 106 & $0.28$ & 4FGL J0608.6+1149 (1.59) & 3FHL J0600.3+1245 (2.59) & -- (--) & -- (--) &    SWIFT J0617.2+09 (3.21) \\
IC20160331 & $151.22^{0.66}_{0.66}$ & $15.48^{0.66}_{0.73}$ & 492 & $0.85$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160410 & $235.63^{1.23}_{1.45}$ & $-4.07^{1.31}_{0.86}$ & 131 & $0.37$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160427 & $240.29^{0.44}_{0.48}$ & $9.71^{0.57}_{0.42}$ & 85 & $0.45$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160510 & $352.88^{1.76}_{1.45}$ & $1.90^{0.75}_{0.67}$ & 208 & $0.39$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160612 & $16.52^{0.88}_{0.18}$ & $4.67^{1.87}_{0.52}$ & 106 & $0.25$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160614 & $214.76^{3.16}_{4.13}$ & $40.82^{3.33}_{3.98}$ & 112 & $0.41$ & 4FGL J1421.1+3859 (1.87) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160615 & $304.32^{1.63}_{1.05}$ & $12.64^{1.33}_{1.34}$ & 150 & $0.41$ & 4FGL J2014.9+1225 (0.61) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160707 & $351.43^{1.54}_{2.29}$ & $0.60^{0.82}_{1.12}$ & 110 & $0.28$ & 4FGL J2326.2+0113 (0.64) & -- (--) & -- (--) & -- (--) &    SWIFT J2318.9+00 (1.74) \\
IC20160720 & $60.25^{10.72}_{8.88}$ & $29.23^{5.32}_{5.87}$ & 108 & $0.37$ & 4FGL J0358.1+2850 (0.74) & 3FHL J0409.4+3201 (3.34) & -- (--) & -- (--) &    SWIFT J0355.5+31 (2.19) \\
IC20160727 & $113.12^{1.93}_{1.54}$ & $14.67^{1.08}_{1.12}$ & 105 & $0.30$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160731 & $214.58^{0.53}_{0.57}$ & $-0.30^{0.45}_{0.67}$ & 98 & $0.44$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160731 & $312.63^{3.74}_{3.21}$ & $20.07^{2.56}_{2.13}$ & 118 & $0.39$ & 4FGL J2043.9+2051 (1.73) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160806 & $122.78^{0.88}_{1.23}$ & $-0.71^{0.56}_{0.56}$ & 219 & $0.58$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20160812 & $86.99^{15.29}_{15.29}$ & $48.83^{9.95}_{10.00}$ & 160 & $0.53$ & 4FGL J0553.5+4810 (1.14) & 3FHL J0533.3+4822 (2.45) & -- (--) & -- (--) &    SWIFT J0547.3+50 (1.83) \\
IC20160814 & $200.04^{3.12}_{2.68}$ & $-32.13^{1.75}_{1.24}$ & 263 & $0.61$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J1325.2-32 (1.25) \\
IC20160924 & $241.13^{4.92}_{5.89}$ & $1.34^{3.40}_{2.80}$ & 191 & $0.51$ & 4FGL J1608.4+0055 (1.07) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20161001 & $192.57^{2.50}_{2.07}$ & $37.12^{1.51}_{2.49}$ & 204 & $0.64$ & 4FGL J1249.8+3707 (0.09) & 3FHL J1249.8+3708 (0.1) & -- (--) & -- (--) & -- (--) \\
IC20161012 & $190.06^{2.20}_{4.04}$ & $-7.48^{2.18}_{2.98}$ & 759 & $0.25$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J1239.6-05 (2.14) \\
IC20161021 & $121.42^{2.64}_{2.90}$ & $23.72^{1.93}_{2.02}$ & 135 & $0.43$ & 4FGL J0803.0+2439 (1.12) & -- (--) & -- (--) & -- (--) &    SWIFT J0800.5+23 (1.34) \\
IC20161027 & $119.00^{2.94}_{2.24}$ & $1.53^{2.32}_{2.39}$ & 155 & $0.38$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20161103 & $40.87^{1.05}_{0.57}$ & $12.52^{1.15}_{0.61}$ & 85 & $0.31$ & 4FGL J0244.7+1316 (0.82) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20161117 & $78.66^{1.85}_{1.93}$ & $1.60^{1.90}_{1.79}$ & 190 & $0.50$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20161125 & $140.01^{2.15}_{1.19}$ & $-0.11^{0.75}_{0.86}$ & 161 & $0.40$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20161127 & $257.55^{36.46}_{29.23}$ & $73.27^{5.71}_{9.96}$ & 139 & $0.45$ & 4FGL J1651.6+7219 (1.66) & 3FHL J1651.6+7219 (1.66) & -- (--) & -- (--) &    SWIFT J1643.2+70 (3.37) \\
IC20161210 & $46.36^{2.37}_{0.92}$ & $15.25^{0.93}_{1.08}$ & 80 & $0.38$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20161224 & $61.79^{2.50}_{2.37}$ & $17.78^{1.46}_{1.56}$ & 139 & $0.42$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0413.3+16 (1.69) \\
IC20170105 & $309.95^{5.01}_{7.56}$ & $8.16^{2.00}_{3.34}$ & 198 & $0.54$ & 4FGL J2035.3+0557 (2.46) & -- (--) & -- (--) & -- (--) &    SWIFT J2033.1+09 (2.41) \\
IC20170206 & $180.35^{5.23}_{3.82}$ & $33.20^{1.85}_{2.16}$ & 135 & $0.46$ & 4FGL J1205.8+3321 (0.94) & -- (--) & -- (--) & -- (--) &    SWIFT J1207.5+33 (1.44) \\
IC20170208 & $99.67^{2.59}_{3.30}$ & $16.84^{1.60}_{1.55}$ & 151 & $0.43$ & 4FGL J0633.9+1746 (1.47) & 3FHL J0633.9+1746 (1.47) & 3HWC J0634+165 (1.14) & Geminga Pulsar (1.47) & -- (--) \\
IC20170208 & $92.81^{1.23}_{1.05}$ & $4.59^{0.94}_{1.16}$ & 133 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170227 & $205.09^{1.89}_{3.96}$ & $4.26^{1.09}_{1.12}$ & 108 & $0.27$ & 4FGL J1342.7+0505 (1.02) & -- (--) & -- (--) & -- (--) &    SWIFT J1338.2+04 (0.59) \\
IC20170308 & $155.35^{2.02}_{1.19}$ & $5.53^{0.98}_{0.90}$ & 107 & $0.25$ & 4FGL J1019.7+0511 (0.53) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170321 & $98.26^{1.32}_{0.92}$ & $-15.06^{1.04}_{1.20}$ & 231 & $0.24$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170422 & $240.95^{3.34}_{5.71}$ & $5.53^{0.83}_{1.01}$ & 161 & $0.39$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170427 & $5.32^{4.48}_{5.27}$ & $-0.60^{1.75}_{1.23}$ & 155 & $0.38$ & 4FGL J0022.0+0006 (0.74) & 3FHL J0022.0+0006 (0.73) & -- (--) & -- (--) &    SWIFT J0009.4-00 (3.02) \\
IC20170514 & $311.97^{2.20}_{1.23}$ & $18.60^{2.10}_{1.10}$ & 109 & $0.34$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170514 & $227.37^{1.23}_{1.10}$ & $30.65^{1.40}_{0.99}$ & 174 & $0.55$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170527 & $178.59^{2.77}_{3.47}$ & $26.49^{3.82}_{3.45}$ & 124 & $0.42$ & 4FGL J1148.5+2629 (1.3) & 3FHL J1152.1+2837 (2.19) & -- (--) & TON 0599 (2.98) & -- (--) \\
IC20170621 & $74.97^{7.25}_{7.78}$ & $25.08^{5.57}_{6.20}$ & 109 & $0.37$ & 4FGL J0501.0+2424 (0.72) & 3FHL J0501.0+2425 (0.71) & -- (--) & VER J0521+211 (6.34) &    SWIFT J0502.4+24 (0.68) \\
IC20170626 & $280.99^{3.03}_{1.63}$ & $8.80^{1.13}_{0.90}$ & 201 & $0.55$ & 4FGL J1846.3+0919 (0.8) & 3FHL J1846.4+0919 (0.81) & -- (--) & -- (--) & -- (--) \\
IC20170704 & $230.45^{1.67}_{1.71}$ & $23.36^{1.10}_{0.89}$ & 195 & $0.60$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170717 & $208.39^{1.67}_{1.19}$ & $25.16^{1.41}_{1.35}$ & 534 & $0.87$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170803 & $1.10^{4.48}_{1.76}$ & $4.63^{0.41}_{0.41}$ & 214 & $0.56$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170809 & $21.27^{0.75}_{1.05}$ & $-2.28^{0.60}_{0.67}$ & 226 & $0.60$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170819 & $26.98^{1.85}_{3.03}$ & $18.88^{1.11}_{1.10}$ & 167 & $0.51$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20170824 & $41.92^{3.03}_{3.56}$ & $12.37^{1.46}_{1.30}$ & 175 & $0.49$ & 4FGL J0244.7+1316 (1.15) & -- (--) & -- (--) & -- (--) &    SWIFT J0248.3+12 (0.38) \\
IC20170922 & $77.43^{1.14}_{0.75}$ & $5.79^{0.64}_{0.41}$ & 264 & $0.63$ & 4FGL J0509.4+0542 (0.11) & 3FHL J0509.4+0542 (0.11) & -- (--) & TXS 0506+056 (0.12) & -- (--) \\
IC20170923 & $173.45^{2.37}_{2.55}$ & $-2.54^{0.90}_{1.31}$ & 202 & $0.56$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20171006 & $132.63^{1.41}_{2.24}$ & $17.23^{1.06}_{0.66}$ & 118 & $0.37$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20171015 & $162.91^{2.99}_{1.71}$ & $-15.48^{1.62}_{1.98}$ & 72 & $0.55$ & -- (--) & -- (--) & -- (--) & -- (--) &   SWIFT J1051.2-170 (1.58) \\
IC20171028 & $294.52^{3.56}_{3.38}$ & $2.05^{2.20}_{3.21}$ & 133 & $0.34$ & 4FGL J1927.5+0154 (2.65) & 3FHL J1927.5+0153 (2.64) & -- (--) & -- (--) & -- (--) \\
IC20171106 & $340.14^{0.62}_{0.62}$ & $7.44^{0.30}_{0.26}$ & 1573 & $0.97$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20171108 & $269.65^{0.22}_{0.18}$ & $-20.70^{0.16}_{0.16}$ & 20310 & $0.18$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180117 & $206.10^{1.19}_{1.14}$ & $3.92^{0.71}_{0.78}$ & 85 & $0.42$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180123 & $77.12^{2.50}_{2.90}$ & $8.01^{0.41}_{0.49}$ & 416 & $0.79$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180125 & $207.51^{1.01}_{0.57}$ & $23.77^{0.57}_{0.57}$ & 110 & $0.36$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180205 & $17.40^{1.36}_{0.92}$ & $-10.54^{0.76}_{0.72}$ & 113 & $0.23$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180213 & $66.97^{2.46}_{2.59}$ & $6.09^{1.95}_{1.72}$ & 111 & $0.27$ & 4FGL J0427.3+0504 (1.02) & -- (--) & -- (--) & -- (--) &    SWIFT J0427.0+07 (1.27) \\
IC20180228 & $294.79^{1.85}_{1.71}$ & $26.40^{0.79}_{1.12}$ & 124 & $0.42$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180313 & $287.18^{0.75}_{2.46}$ & $5.53^{0.34}_{0.26}$ & 160 & $0.39$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180314 & $58.71^{1.89}_{1.67}$ & $0.78^{1.01}_{1.01}$ & 145 & $0.36$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180316 & $271.71^{1.19}_{3.43}$ & $-1.42^{1.23}_{1.27}$ & 156 & $0.39$ & 4FGL J1759.0-0107 (1.97) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180410 & $218.50^{0.79}_{1.27}$ & $0.56^{0.75}_{0.71}$ & 234 & $0.60$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180417 & $305.73^{3.60}_{1.58}$ & $-4.41^{0.67}_{0.75}$ & 202 & $0.58$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180528 & $312.14^{1.41}_{2.02}$ & $0.30^{0.86}_{1.45}$ & 110 & $0.28$ & 4FGL J2049.7-0036 (0.97) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180608 & $69.08^{1.63}_{1.41}$ & $-1.08^{0.78}_{0.78}$ & 158 & $0.40$ & 4FGL J0436.2-0038 (0.43) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180612 & $338.69^{5.10}_{5.71}$ & $3.73^{2.81}_{3.70}$ & 107 & $0.25$ & 4FGL J2226.6+0210 (2.56) & 3FHL J2227.8+0036 (3.56) & -- (--) & -- (--) &    SWIFT J2235.7+01 (2.12) \\
IC20180613 & $38.06^{5.84}_{4.26}$ & $11.53^{4.15}_{4.91}$ & 155 & $0.41$ & 4FGL J0231.8+1322 (1.84) & 3FHL J0233.5+0657 (4.58) & -- (--) & -- (--) &    SWIFT J0245.2+10 (3.29) \\
IC20180728 & $74.14^{0.44}_{0.35}$ & $-17.74^{0.51}_{0.59}$ & 16952 & $0.18$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180807 & $100.37^{4.00}_{5.05}$ & $11.15^{2.98}_{2.12}$ & 106 & $0.28$ & 4FGL J0642.4+1048 (0.41) & -- (--) & 3HWC J0631+107 (2.58) & -- (--) &    SWIFT J0630.9+11 (2.68) \\
IC20180908 & $144.98^{1.49}_{2.20}$ & $-2.39^{1.16}_{1.12}$ & 144 & $0.30$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180909 & $141.37^{1.05}_{1.27}$ & $26.94^{0.88}_{1.00}$ & 171 & $0.53$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20180919 & $258.40^{1.49}_{1.49}$ & $32.84^{0.94}_{0.75}$ & 144 & $0.48$ & 4FGL J1714.6+3228 (0.43) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20181008 & $77.08^{2.68}_{3.56}$ & $1.23^{1.23}_{1.16}$ & 108 & $0.27$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20181014 & $225.22^{1.36}_{2.64}$ & $-34.95^{1.22}_{1.79}$ & 62 & $0.39$ & 4FGL J1505.0-3433 (0.94) & 3FHL J1457.5-3538 (0.98) & -- (--) & -- (--) & -- (--) \\
IC20181023 & $270.18^{1.89}_{1.71}$ & $-8.42^{1.13}_{1.55}$ & 237 & $0.15$ & 4FGL J1804.4-0852 (1.03) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20181023 & $78.27^{1.76}_{0.92}$ & $21.54^{0.96}_{0.93}$ & 136 & $0.43$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20181114 & $6.02^{1.63}_{2.24}$ & $18.84^{0.87}_{0.98}$ & 145 & $0.44$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20181120 & $25.71^{5.54}_{5.27}$ & $11.72^{2.41}_{4.50}$ & 188 & $0.54$ & 4FGL J0150.9+1230 (2.13) & 3FHL J0159.5+1047 (4.2) & -- (--) & -- (--) & -- (--) \\
IC20181120 & $324.58^{7.74}_{9.04}$ & $51.74^{6.75}_{9.48}$ & 173 & $0.57$ & 4FGL J2123.9+5158 (2.23) & -- (--) & -- (--) & -- (--) &    SWIFT J2133.6+51 (0.94) \\
IC20181121 & $132.19^{7.34}_{6.99}$ & $32.93^{4.19}_{3.57}$ & 209 & $0.65$ & 4FGL J0850.5+3455 (2.03) & 3FHL J0850.6+3454 (2.01) & -- (--) & -- (--) &    SWIFT J0848.1+34 (1.81) \\
IC20181212 & $316.41^{1.85}_{2.02}$ & $-31.00^{1.68}_{1.58}$ & 162 & $0.46$ & 4FGL J2112.5-3043 (1.51) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190113 & $56.91^{1.63}_{1.41}$ & $-0.82^{0.75}_{0.82}$ & 156 & $0.39$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190124 & $307.44^{0.53}_{1.14}$ & $-32.22^{0.96}_{0.31}$ & 157 & $0.74$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190201 & $245.08^{0.75}_{0.88}$ & $38.78^{0.77}_{0.67}$ & 163 & $0.53$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190214 & $228.25^{0.79}_{0.53}$ & $-4.14^{0.37}_{0.30}$ & 348 & $0.74$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190221 & $268.59^{1.41}_{1.58}$ & $-17.00^{1.24}_{0.51}$ & 56 & $0.55$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190223 & $155.21^{0.70}_{0.66}$ & $19.67^{0.28}_{0.44}$ & 168 & $0.51$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190317 & $81.25^{5.89}_{5.98}$ & $3.21^{3.93}_{4.07}$ & 108 & $0.26$ & 4FGL J0521.6+0103 (2.31) & 3FHL J0521.6+0104 (2.3) & -- (--) & -- (--) & -- (--) \\
IC20190410 & $310.61^{3.30}_{3.65}$ & $12.22^{2.84}_{2.28}$ & 105 & $0.28$ & 4FGL J2044.0+1036 (1.66) & 3FHL J2035.5+1056 (2.12) & -- (--) & -- (--) & -- (--) \\
IC20190413 & $219.33^{0.70}_{1.32}$ & $11.72^{0.72}_{0.72}$ & 107 & $0.29$ & 4FGL J1438.6+1205 (0.49) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190413 & $245.57^{1.23}_{1.49}$ & $21.98^{1.21}_{1.44}$ & 115 & $0.38$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190415 & $154.86^{2.94}_{4.70}$ & $5.27^{2.48}_{1.95}$ & 117 & $0.30$ & 4FGL J1019.7+0511 (0.11) & 3FHL J1016.0+0512 (0.85) & -- (--) & -- (--) & -- (--) \\
IC20190422 & $166.90^{3.21}_{3.03}$ & $17.39^{2.00}_{2.56}$ & 170 & $0.51$ & 4FGL J1112.4+1751 (1.24) & 3FHL J1107.8+1501 (2.36) & -- (--) & -- (--) & -- (--) \\
IC20190503 & $120.19^{0.66}_{0.66}$ & $6.43^{0.68}_{0.75}$ & 142 & $0.34$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190504 & $65.17^{1.67}_{1.14}$ & $-37.26^{0.61}_{1.09}$ & 55 & $0.39$ & 4FGL J0420.3-3745 (0.5) & 3FHL J0420.4-3744 (0.48) & -- (--) & -- (--) & -- (--) \\
IC20190515 & $127.88^{0.79}_{0.83}$ & $12.60^{0.50}_{0.46}$ & 457 & $0.82$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190613 & $312.19^{0.66}_{0.79}$ & $26.57^{0.75}_{0.71}$ & 195 & $0.61$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20190619 & $343.52^{4.13}_{3.16}$ & $10.28^{2.02}_{2.76}$ & 199 & $0.55$ & -- (--) & -- (--) & -- (--) & -- (--) &   SWIFT J2254.2+114 (1.49) \\
IC20190629 & $29.12^{39.68}_{118.65}$ & $84.56^{4.66}_{4.40}$ & 109 & $0.34$ & 4FGL J0250.6+8435 (1.28) & 3FHL J0249.7+8434 (1.26) & -- (--) & -- (--) &    SWIFT J0048.9+82 (2.76) \\
IC20190704 & $161.81^{2.15}_{3.91}$ & $26.90^{1.94}_{1.91}$ & 155 & $0.49$ & 4FGL J1049.8+2741 (0.97) & -- (--) & -- (--) & -- (--) &    SWIFT J1046.8+25 (0.98) \\
IC20190712 & $76.64^{5.23}_{6.99}$ & $12.75^{4.79}_{2.82}$ & 109 & $0.30$ & 4FGL J0502.5+1340 (1.34) & 3FHL J0458.0+1151 (2.25) & -- (--) & -- (--) &    SWIFT J0510.7+16 (3.9) \\
IC20190730 & $226.14^{1.27}_{1.98}$ & $10.77^{1.03}_{1.17}$ & 298 & $0.67$ & 4FGL J1504.4+1029 (0.27) & 3FHL J1504.3+1030 (0.27) & -- (--) & -- (--) &    SWIFT J1504.2+10 (0.35) \\
IC20190819 & $148.54^{2.29}_{3.30}$ & $1.45^{0.93}_{0.75}$ & 113 & $0.29$ & -- (--) & 3FHL J0946.2+0104 (2.01) & -- (--) & -- (--) & -- (--) \\
IC20190922 & $167.30^{2.81}_{2.72}$ & $-22.27^{3.39}_{3.31}$ & 3114 & $0.20$ & 4FGL J1103.6-2329 (1.77) & 3FHL J1103.6-2328 (1.77) & -- (--) & 1ES 1101-232 (1.78) &    SWIFT J1103.5-23 (1.78) \\
IC20190922 & $5.71^{1.19}_{1.27}$ & $-1.53^{0.90}_{0.78}$ & 187 & $0.50$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20191001 & $313.99^{6.94}_{2.46}$ & $12.79^{1.65}_{1.64}$ & 218 & $0.59$ & 4FGL J2052.7+1218 (0.91) & -- (--) & -- (--) & -- (--) &    SWIFT J2106.0+14 (2.79) \\
IC20191119 & $229.31^{5.49}_{4.97}$ & $3.77^{2.47}_{2.24}$ & 177 & $0.45$ & 4FGL J1521.1+0421 (1.15) & 3FHL J1512.2+0203 (2.11) & -- (--) & -- (--) &    SWIFT J1521.8+03 (1.18) \\
IC20191122 & $27.03^{1.98}_{2.72}$ & $0.07^{1.08}_{1.57}$ & 127 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20191204 & $80.16^{2.42}_{1.98}$ & $2.87^{1.05}_{0.97}$ & 130 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20191215 & $286.83^{2.27}_{1.92}$ & $58.45^{2.08}_{1.86}$ & 133 & $0.48$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20191231 & $48.47^{5.98}_{7.65}$ & $20.11^{4.48}_{3.73}$ & 156 & $0.46$ & 4FGL J0312.7+2012 (0.28) & 3FHL J0312.7+2013 (0.28) & -- (--) & RBS 0413 (1.94) &    SWIFT J0256.2+19 (4.23) \\
IC20200109 & $165.45^{3.60}_{4.39}$ & $11.80^{1.18}_{1.29}$ & 375 & $0.77$ & 4FGL J1103.0+1157 (0.36) & 3FHL J1103.1+1156 (0.35) & -- (--) & -- (--) &    SWIFT J1100.9+11 (0.7) \\
IC20200117 & $116.02^{0.79}_{1.19}$ & $29.18^{0.86}_{0.81}$ & 108 & $0.38$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0744.0+29 (0.09) \\
IC20200120 & $67.41^{0.40}_{0.31}$ & $-14.59^{0.23}_{0.27}$ & 6055 & $0.31$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200410 & $242.58^{10.20}_{10.20}$ & $11.61^{7.83}_{6.19}$ & 110 & $0.30$ & 4FGL J1608.7+1029 (1.18) & 3FHL J1603.8+1103 (1.69) & -- (--) & PG 1553+113 (3.6) &    SWIFT J1608.8+12 (0.78) \\
IC20200421 & $87.93^{3.43}_{2.81}$ & $8.23^{2.08}_{1.81}$ & 127 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200425 & $99.97^{4.76}_{3.00}$ & $53.72^{2.25}_{1.69}$ & 135 & $0.48$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0645.9+53 (1.14) \\
IC20200512 & $295.18^{1.67}_{2.24}$ & $15.79^{1.24}_{1.28}$ & 109 & $0.32$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200523 & $338.64^{9.98}_{6.02}$ & $1.75^{1.79}_{3.51}$ & 105 & $0.25$ & 4FGL J2227.9+0036 (2.01) & 3FHL J2227.8+0036 (2.02) & -- (--) & -- (--) &    SWIFT J2235.7+01 (0.3) \\
IC20200530 & $255.37^{2.46}_{2.55}$ & $26.61^{2.32}_{3.25}$ & 82 & $0.59$ & 4FGL J1702.2+2642 (0.2) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200614 & $33.84^{4.79}_{6.37}$ & $31.61^{2.71}_{2.25}$ & 115 & $0.41$ & 4FGL J0220.2+3246 (1.57) & 3FHL J0203.8+3044 (2.61) & -- (--) & -- (--) & -- (--) \\
IC20200615 & $142.95^{1.14}_{1.41}$ & $3.66^{1.16}_{1.01}$ & 496 & $0.83$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200620 & $162.11^{0.62}_{0.92}$ & $11.95^{0.61}_{0.46}$ & 114 & $0.33$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200806 & $157.25^{1.17}_{0.87}$ & $47.75^{0.64}_{0.59}$ & 107 & $0.40$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200911 & $51.11^{4.39}_{10.99}$ & $38.11^{2.31}_{1.97}$ & 111 & $0.41$ & -- (--) & -- (--) & -- (--) & -- (--) &    SWIFT J0333.3+37 (1.94) \\
IC20200916 & $109.78^{1.05}_{1.41}$ & $14.36^{0.85}_{0.81}$ & 110 & $0.32$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200921 & $195.29^{2.33}_{1.71}$ & $26.24^{1.46}_{1.73}$ & 117 & $0.41$ & -- (--) & 3FHL J1303.0+2435 (1.7) & -- (--) & -- (--) & -- (--) \\
IC20200926 & $96.46^{0.70}_{0.53}$ & $-4.33^{0.60}_{0.75}$ & 670 & $0.44$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200926 & $184.75^{3.65}_{1.54}$ & $32.93^{1.16}_{0.88}$ & 121 & $0.43$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20200929 & $29.53^{0.53}_{0.53}$ & $3.47^{0.71}_{0.34}$ & 183 & $0.47$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201007 & $265.17^{0.48}_{0.48}$ & $5.34^{0.30}_{0.19}$ & 683 & $0.89$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201014 & $221.22^{0.97}_{1.19}$ & $14.44^{0.66}_{0.46}$ & 147 & $0.41$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201021 & $260.82^{1.71}_{1.67}$ & $14.55^{1.31}_{0.69}$ & 105 & $0.30$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201114 & $105.73^{0.92}_{1.27}$ & $5.87^{1.05}_{1.01}$ & 214 & $0.56$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201115 & $195.12^{1.23}_{1.45}$ & $1.38^{1.27}_{1.08}$ & 177 & $0.46$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201120 & $307.66^{5.19}_{5.68}$ & $40.72^{5.02}_{2.75}$ & 154 & $0.50$ & 4FGL J2032.6+4053 (0.41) & 3FHL J2028.6+4110 (0.58) & 3HWC J2031+415 (0.82) & LHAASO J2032+410 (0.44) &    SWIFT J2032.5+40 (0.41) \\
IC20201130 & $30.54^{1.10}_{1.27}$ & $-12.10^{1.14}_{1.11}$ & 203 & $0.15$ & 4FGL J0206.4-1151 (1.07) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201209 & $6.86^{1.01}_{1.19}$ & $-9.25^{0.94}_{1.10}$ & 419 & $0.19$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201221 & $261.69^{2.28}_{2.46}$ & $41.81^{1.25}_{1.14}$ & 175 & $0.56$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\
IC20201222 & $206.37^{0.88}_{0.75}$ & $13.44^{0.54}_{0.34}$ & 186 & $0.53$ & -- (--) & -- (--) & -- (--) & -- (--) & -- (--) \\

